A posteriori error estimates and adaptivity for locally conservative methods. Inexpensive implementation and evaluation, polytopal meshes, iterative linearization and algebraic solvers, and applications to complex porous media flows

A posteriori estimates give bounds on the error between the unknown solution of a partial differential equation and its numerical approximation. We present here the methodology based on H1-conforming potential and H(div)-conforming equilibrated flux reconstructions, where the error bounds are guaranteed and fully computable. We consider any lowest-order locally conservative method of the finite volume type and treat general polytopal meshes. We start by a pure diffusion problem and first address the discretization error. We then progressively pass to more complicated model problems, up to complex multiphase multicomponent flow in porous media, and also take into account the errors arising in iterative linearization of nonlinear problems and in algebraic resolution of systems of linear algebraic equations. We focus on the ease of implementation and evaluation of the estimates. In particular, the evaluation of our estimates is explicit and inexpensive, since it merely consists in some local matrix-vector multiplications. Here, on each mesh element, the matrices are either directly inherited from the given numerical method, or easily constructed from the element geometry, while the vectors are the algebraic unknowns of the flux and potential approximations on the given element. Our mtehodology leads to an easy-to-implement and fast-to-run adaptive algorithm with guaranteed overall precision, adaptive stopping criteria for nonlinear and linear solvers, and adaptive space and time mesh refinements and derefinements. Progressively along the theoretical exposition, numerical experiments on academic benchmarks as well as on real-life problems in two and three space dimensions illustrate the performance of the derived methodology. The presentation is largely self-standing, developing all the details and recalling all necessary basic notions.

==> Figs/LShape.tex <==
N          l2        error   estimate    sol      grad   relativeErr relativeEst effId
2700    0.0005287  0.019418 0.0261825  1.04129   1.35427    0.01433    0.01933 1.34836  
10800   0.0002126  0.012233 0.0165004  1.04129   1.35427    0.00903    0.01218 1.34884
43200   8.504e-05  0.007706 0.0103962  1.04129   1.35427    0.00569    0.00767 1.34910      

==> Figs/LShapeNL.tex <==
fact     error      estimate    index
1e1      0.02084     0.028241    1.355
1e2      0.02297     0.031127    1.355
1e3      0.02321     0.031470    1.355
1e4      0.02323     0.031497    1.355
1e5      0.02323     0.031497    1.355
1e6      0.02323     0.031497    1.355


==> Figs/LShape_nb_iter.tex <==
fact    classic     adaptive
1e1     17          6
1e2     19          8
1e3     19          8
1e4     19          8
1e5     19          8
1e6     19          8

==> Figs/Lshape_iter.tex <==
iter   estimate        linEst          linErr
1      0.0152555       1.35444         0.00273150632075092  
2      0.377743        0.51422         0.01687745781405  
3      0.0185568       0.509583        0.000691693788253631  
4      0.0501492       0.0437614       0.000860131013830517  
5      0.0206323       0.0433356       0.000127945304350981  
6      0.0248501       0.0047324       0.000115569509245781  
7      0.020947        0.00537146      2.39701786846096e-05  
8      0.021517        0.000491099     1.95404877860202e-05  
9      0.0209005       0.000788214     3.96496799187309e-06  
10     0.0209541       5.72348e-05     3.17391528487607e-06  
11     0.0208591       0.000117604     6.11738535691112e-07  
12     0.020859        1.61975e-05     4.94561183334594e-07  
13     0.0208446       1.80057e-05     9.98960757220402e-08  
14     0.020843        4.33672e-06     7.66523698407532e-08  
15     0.0208408       2.90468e-06     1.90239130868413e-08  
16     0.0208403       9.86298e-07     1.23616327077025e-08  
17     0.02084         5.01272e-07     3.9348099155847e-09  


==> Figs/relative.tex <==
N	      error			estimate     new        modif
7290	0.01759			0.03215      0.03332	0.03281	
28656	0.01208			0.02192      0.02325    0.02323
113724	0.00841			0.01546      0.01609    0.01607
450846	0.00570			0.01042      0.01086    0.01081

==> Figs/relativeAd.tex <==
N       error		new		modif	estimate
7290	0.01762	  0.03332  0.03329	0.03221		
13194	0.01327	  0.02182  0.02168  0.02204
16758	0.00843	  0.01306  0.01307	0.01313
24750	0.00612   0.00878  0.00878	0.00858



==> Figs/res-convergence.tex <==
N         e           error     estimate    grad      relativeErr relativeEst effId 
2500    0.00096022  0.187924    0.252776    1.80639     0.10403    0.13993    1.3451 
10000   0.00023820  0.080766    0.094125    1.80639     0.04471    0.05210    1.1654 
40000   5.9436e-05  0.032923    0.037619    1.80639     0.01822    0.02082    1.1424  
160000  1.4852e-05  0.013217    0.014817    1.80639     0.00731    0.00820    1.1211 

==> Figs/smooth_iter.tex <==
fact    classic     adaptive
1e1     22          7
1e2     22          9
1e3     25          11
1e4     24          12
1e5     24          12
1e6     24          12

==> Figs/smooth_sol_iterations.tex <==
iter    estimate    linEst      linErr
1   0.3515          0.635685978     0.00488493409012246  
2   0.7125          0.477738361     0.0363173291393307 
3   0.2042          0.459570230     0.00270443609163948
4   0.2030          0.105856487     0.00465425294393055
5   0.2030          0.101873370     0.00104585135131234
6   0.2031          0.020990533     0.000995525982071665
7   0.2022          0.022775891     0.000363462295230952
8   0.2025          0.003300901     0.000252089722533724 
9   0.2023          0.004728124     8.95699879135772e-05
10  0.2019          0.000692667     5.38799611921888e-05 
11  0.2016          0.000962690     1.80223105180065e-05
12  0.2016          0.000253635     9.88464358315917e-06 
13  0.2015          0.000202905     3.66415176803706e-06
14  0.2015          0.000084403     1.6791791072397e-06
15  0.2015          0.000045765     9.05288593168526e-07
16  0.2015          0.000024836     3.10283150914203e-07
17  0.2015          0.000011244     2.43671224079373e-07
18  0.2015          0.000006846     7.21600098021785e-08
19  0.2015          0.000002991     6.33990138773096e-08
20  0.2015          0.000001840     1.98268203156667e-08
21  0.2015          0.000000834     1.58840618994112e-08
22  0.2015          0.000000493     5.79907145373147e-09

==> Figs/smooth_sol_sharpness.tex <==
fact    error   estimate    index
1e1     0.17149  0.2015      1.1755
1e2     0.18009  0.2132      1.1841
1e3     0.18159  0.2150      1.1841
1e4     0.18171  0.2152      1.1847
1e5     0.18176  0.2153      1.1847
1e6     0.18176  0.2153      1.1847
